On multivariate polynomials achievable with quantum signal processing

Quantum signal processing (QSP) is a framework which was proven to unify and simplify a large number of known quantum algorithms, as well as discovering new ones. QSP allows one to transform a signal embedded in a given unitary using polynomials. Characterizing which polynomials can be achieved with QSP protocols is an important part of the power of this technique, and while such a characterization is well-understood in the case of univariate signals, it is unclear which multivariate polynomials can be constructed when the signal is a vector, rather than a scalar. This work uses a slightly different formalism than what is found in the literature, and uses it to find simpler necessary conditions for decomposability, as well as a sufficient condition -- the first, to the best of our knowledge, proven for a (generally inhomogeneous) multivariate polynomial in the context of quantum signal processing.

==> contents/apx-3d-implementation.tex <==
\section{Implementation of Protocol \ref{def:three-dimensional-qsp}}
In this appendix we show how to implement Protocol~\ref{def:three-dimensional-qsp} by obtaining a phase factor decomposition for $SU(3)$ similar to what we have for $SU(2)$. Let us start from a general single-qubit QSP protocol in one variable:
\begin{align*}
    A_0 \Tilde{w} A_1 \Tilde{w} \cdots \Tilde{w} A_{n-1} \Tilde{w} A_n \ .
\end{align*}
As shown in Section~\ref{sec:univariate-qsp}, we can decompose $A_k = e^{i \alpha_k Z} e^{i \phi_k X} e^{i \beta_k Z}$ and, by the fact that $\Tilde{w}$ commutes with $Z$, the protocol can be simply rewritten as
\begin{align*}
    e^{i \alpha_0 Z} e^{i \phi_0 X} e^{i (\beta_0 + \alpha_1) Z} \Tilde{w}\  e^{i \phi_1 X} e^{i (\beta_1 + \alpha_2) Z} \Tilde{w} \cdots \Tilde{w}\  e^{i \phi_n X} e^{i \beta_n Z}
\end{align*}
This is generalized QSP~\cite{motlaghGeneralizedQuantumSignal2024} (up to a global phase), and can construct any pair of univariate polynomials. We carry out a similar decomposition using the Sinkhorn normal form for unitary matrices~\cite{idelSinkhornNormalForm2015}. A unitary $V_n \in SU(n)$ can be decomposed as follows
\begin{align*}
    V_n =
    \begin{bmatrix}
        e^{i\alpha_1} & & \\
        & e^{i\alpha_2} & \\
        & & e^{-i(\alpha_1 + \alpha_2)}
    \end{bmatrix}
    Q_3
    \begin{bmatrix}
        e^{i\phi} & \\
        & e^{-i\phi} V_2
    \end{bmatrix}
    Q_3^{\dag}
    \begin{bmatrix}
        e^{i\beta_1} & & \\
        & e^{i\beta_2} & \\
        & & e^{-i(\beta_1 + \beta_2)}
    \end{bmatrix}
\end{align*}
for some $V_2 \in SU(2)$, where $Q_3$ is the quantum Fourier transform over $\Z_3$. This is parameterized by $8$ phase factors, if we include the Euler decomposition of $V_2$. By calling $R(\vec{\alpha})$ the matrix on the left, and $S(\phi, V_2)$ the matrix in the middle with the QFT, Protocol~\ref{def:three-dimensional-qsp} can be simplified just like the single-qubit case above:
\begin{align*}
    R(\lambda_1, \lambda_2) S(\phi_0, U_0) R(\vec{\psi}_0) \Tilde{W} S(\phi_1, U_1) R(\vec{\psi}_1) \Tilde{W} \cdots \Tilde{W} S(\phi_n, U_n) R(\vec{\psi}_n)
\end{align*}

==> libs/handouts.tex <==
\usepackage{environ}

\newcommand{\handout}[5]{
   \noindent
   \begin{center}
        \framebox{\vbox{
            \hbox to 0.95\textwidth { {\bf #1} \hfill #2 }
            \vspace{5mm}
            \hbox to 0.95\textwidth { {\Large \hfill #5  \hfill} }
            \vspace{6mm}
            \hbox to 0.95\textwidth { {\it #3 \hfill #4} }
      }
   }
   \end{center}
   \vspace*{4mm}
}

\newcommand{\handoutCourse}[1]{\newcommand{\hoCourse}{#1}}
\newcommand{\handoutLecturers}[1]{\newcommand{\hoLecturers}{#1}}

\newcommand{\syllabus}{\handout{\hoCourse}{\hoLecturers}{}{}{Course Information}}
\newcommand{\lecture}[1]{\handout{\hoCourse}{\hoLecturers}{}{}{#1}}
\newcommand{\exercise}[1]{\handout{\hoCourse}{\hoLecturers}{}{}{Exercise Sheet #1}}
\newcommand{\assignment}[1]{\handout{\hoCourse}{\hoLecturers}{}{}{Assignment #1}}

\newcommand{\makesyllabustitle}{\syllabus}
\newcommand{\makelecturetitle}[1]{\lecture{#1}}
\newcommand{\makeexercisetitle}[1]{\exercise{#1}}
\newcommand{\makeassignmenttitle}[1]{\assignment{#1}}

\newcounter{subtaskc}[section]
\newif\ifinsubtask
\insubtaskfalse

\def\getintosubt@sk{
    \ifinsubtask\else
        \advance\linewidth -\leftmargin
        \advance\leftskip\leftmargin
    \fi
    \global\insubtasktrue
}

\def\outofsubt@sk{
    \ifinsubtask
        \advance\linewidth\leftmargin
        \advance\leftskip-\leftmargin
        \global\insubtaskfalse
    \fi
}

\newcommand{\task}[1]{
    \outofsubt@sk
    \section{#1}
}

\newcommand{\subtask}{
    \vspace*{0.8em}
    \par\vskip0.5ex plus 0.2ex minus0.1ex
    \stepcounter{subtaskc}
    \getintosubt@sk
    {\noindent\llap{(\roman{subtaskc})\hskip 0.5em}}
}

\newcommand{\nosubtask}{
    \outofsubt@sk
    \vspace*{1em}
}

\newif\ifsolutionshidden
\solutionshiddenfalse

\newcommand{\showsolutions}{\global\solutionshiddenfalse}
\newcommand{\hidesolutions}{\global\solutionshiddentrue}

\NewEnviron{solution}{
    \ifsolutionshidden\else
        \noindent
        \begin{center}
            \vspace*{-0.8em}
            \setlength\fboxsep{0pt}
            \colorbox{gray!20}{\framebox{
                \vbox{
                    \vspace*{-0.2em}
                    \justify
                    \textbf{Solution.}\ \ \BODY
                    \vspace*{0.8em}
                }
            }}
        \end{center}
    \fi
}

==> libs/slides.tex <==

\def\skiptheoremsetup{}

\usepackage{qrcode}

\newcommand{\hidenavbar}{\def\navbarhidden{}}
\newcommand{\paperuri}[1]{\def\thepaperuri{#1}}

\input{libs/graphics}
\input{libs/math}
\input{libs/complexity}
\input{libs/quantum}
